Reputation Gaming in Stack Overflow

Stack Overflow incentive system awards users with reputation scores to ensure quality. The decentralized nature of the forum may make the incentive system prone to manipulation. This paper offers, for the first time, a comprehensive study of the reported types of reputation manipulation scenarios that might be exercised in Stack Overflow and the prevalence of such reputation gamers by a qualitative study of 1,697 posts from meta Stack Exchange sites. We found four different types of reputation fraud scenarios, such as voting rings where communities form to upvote each other repeatedly on similar posts. We developed algorithms that enable platform managers to automatically identify these suspicious reputation gaming scenarios for review. The first algorithm identifies isolated/semi-isolated communities where probable reputation frauds may occur mostly by collaborating with each other. The second algorithm looks for sudden unusual big jumps in the reputation scores of users. We evaluated the performance of our algorithms by examining the reputation history dashboard of Stack Overflow users from the Stack Overflow website. We observed that around 60-80% of users flagged as suspicious by our algorithms experienced reductions in their reputation scores by Stack Overflow.

==> implications.tex <==
%------------------------------------------
\section{Implications of Findings}\label{sec:implications}
%------------------------------------------
\begin{enumerate}
  \item Community. The fraud users often work in a group to upvote each other.
  \item Jump. The score a fraud user may show a sudden jump unlike to the majority of active users.
\end{enumerate}

The Stack Overflow development team internally develops algorithms to detect voting rings. The algorithms are not shared in the forums. The Stack Overflow admins are provided insights into how such algorithms work. While the admins are not allowed to share those insights in forum posts, they share their opinions in forum posts when other users consult the voting ring scenarios. 
The severity of the fraud activities call for prevention and mitigation measures.
Developers discussed three types of solutions.

\begin{description}
\item[Automated Analysis.]{A group of users always upvoting each other can be detected based on
their usage/navigation patterns. Developers recommend automated clustering to
group users originating from similar network addresses (e.g., same IP/institution). By matching the IP, one
such fraud was tracked to groups of students from a
university~\cite{website:stackoverflow-322114}. StackOverflow
then contacted the chancellor of the university.
The problem is that good users can also share the same IP
(e.g., employees from a company).
}
\item[Support Mechanisms.]{The developers asked for strict background checks to
register, to prevent users from creating multiple fake accounts. They
recommended increased visibility into the voting process and asked for two
versions of StackOverflow: professional vs novice developers. However, with increased difficulty to
participate in forums,
newcomers may feel unwelcome and decide not to use StackOverflow.

}
\item[Community Engagement.]{Developers asked for increased communications with
the moderators and StackOverflow employees. The moderators acknowledged
the challenges that they face in detecting the
frauds. They have more
power than developers, but they cannot see who voted.
This visibility is important to identify fraud patterns. They propose
to engage StackOverflow employees to see those.
}
\end{description}
The following techniques can improve the automated
detection of frauds.
\begin{description}
\item[Social Network Analysis.] The developers in a ring vote
for each other more than they vote for others. We
could create a graph with each developer as a node and an
edge between those who voted for each other.
%The weight of the edge could be the number of times a developer has voted for
% the other.
Social network analysis techniques can be applied on this
graph to identify the developers forming a
ring~\cite{Otte-SocialNetworkAnalysis-JIS2002}.

\item[Time.] The developers in a ring tend to vote within a short
interval of time. By projecting the votes into a time-series,
we can apply techniques from temporal analysis of events in social networks to
detect those patterns~\cite{Ahn-TemporalVisualizationSNA-ICSC2011}.

\item[Content Quality.] The fraud posts are low-quality/spams. Bayesian approaches to detect
spam/junk emails can be adapted to detect such
posts~\cite{Sahami-SpamEmailBaysian-AAAI1998}.
\end{description}


The reputation frauds can harm the forum content quality
and their adoption by others.
%\Foutse{by using items instead of subsections you may save space here....and
% also, we can make this more concise i think since some of the implications mentioned here are quite straightforward...}
%\subsection*{Power Abuse}
%\Foutse{i would rephrase the first sentence!}The biggest impact of reputation
% fraud is that developers can gain reputation underservignly.
A fraud developer with high reputation can promote other frauds and 
influence the future direction of the forums.
An admin in StackOverflow was identified as
using bounty unfairly to promote his friends into the admin level.
\begin{quote}
\it{The bounties were place on three questions by a high rep user to give a
lower rep user the reputation by rewarding existing answers.
This was to assist the lower rep user attain a rep level that
would give that user moderation privileges.} \bf{MSO$_{A,318504}$}
\end{quote}
%\subsection*{Lack of Trust}
%\subsection*{Lack of Visibility}
The frauds can discourage developers' engagement by
promoting bad contents over good contents. A developer, subjected to revenge
voting, was concerned that his posts may not appear in the search results,
due to low/negative scores.
\begin{quote}
\it{If I
"cross" 40 users dumb enough to downvote 2 or 3 of my questions,
my questions will have a 0 score. That is harmful because it would be
like none voted for them, so they won't stand out in searches, and the
content will be less read.} \bf{MSO$_{C,510837}$}
\end{quote}
%
% \begin{quote}
% \it{``I got some mini-revenge (2 or 3 downvotes simultaneously on unrelated
% well-written questions) on specific questions (score was 0 or 1, now it's -1 or
% 0). It has greatly impacted the visibility of those questions. What should I do?''}
% \end{quote}

%\subsection*{Lack of Adoption}
We observed the fraud concerns can fuel a
lack of trust among developers and forum admins. 
\begin{quote}
\it{\ldots it's so bad you don't trust specific moderators to act in a way
that best represents the community they were elected to serve.} \bf{MSE$_{C,333446}$}
\end{quote}
%In the long run, the forums become less useful with more lower quality
% contents.
% The following developer is already concerned with the current contents.
% \begin{quote}
% \it{I remember at the beginning of StackOverflow learning a lot by looking up
% at the questions. Now... well, finding a good question in the most
% popular tags is just hard. I keep trudging through crap.} \bf{MSO$_{A,256304}$}
% \end{quote}

%\Foutse{all these quotes are nice but we never actually showed numbers about
% the magnitude of this problem...any reviewer will question this... if it is in a figure (that i don't see from the tex) then that haven't been discussed in the text, which is a problem!!!}




%\item[Anonymization.] While it is not possible to disclose who voted
%for a post, their identity can be anonymized and then shared to
%facilitate public research. A hash can be created using the various attributes
%of a developer, e.g., her email address and locality.
% Proper security measures can be applied to prevent so that the tracking of
% the actual developer from the hash would be possible only by the StackOverflow employees.
%\end{description}
%
%
% A more sophisticated approach is to include the time of voting into the usage
% clustering as well as the content of the posts. Intuitively, the participants in
% a voting ring upvote in a short period of time. The posts they upvote may also
% be of lower quality and can sometimes be considered as spams. One developer used
% this approach to identify such a scenario.
% \begin{quote}
% \it{The last three questions of this particular user are mediocre at best, yet
% still have received 5-7 upvotes in less than 24 hours after posting. That,
% combined with your observation about his coworker answering the question
% (which is perfectly acceptable under normal circumstances) would be enough
% reason for me to raise a custom moderator flag on one of his posts.}
% \bf{MSO$_{A,338447}$}
% \end{quote} However, the identification of lower quality contents of spams in
% the forum posts is a non-trivial task. Such detection is so far manual in Stack
% Overflow, which is not scalable given the pervasive nature of the problem.



==> methodology.tex <==
%------------------------------------------
\section{Research Methodology}\label{sec:research-method}
%------------------------------------------
In this section, we describe the methodology we followed to conduct the two empirical studies. 
Our first study focuses on understanding the different types of reputation fraud scenarios that can be used to exploit the reputation 
mechanism in Stack Overflow. Our second study focuses on the automatic detection of suspicious users in Stack Overflow who could be potential reputation frauds. 
% In particular, through the two empirical studies, we seek to answer the following research questions:
% \begin{enumerate}[label=\textbf{RQ\arabic*.}, leftmargin=10mm]
%   \item What are the different reputation fraud scenarios reported by developers in Stack Overflow? (Study 1)
%   
%   %\item How are suspicious votings addressed by Stack Overflow?
%   \item Can we automatically detect reputation frauds in Stack Overflow? (Study 2)
%   %\item How do Stack Overflow users behave before and after the removal of their reputation scores?
% \end{enumerate}
In \fig\ref{fig:MethodologyOverall}, we show the major steps we followed to conduct the two studies. We describe the steps below.


\subsection{Study 1. Reputation Fraud Scenarios}
Our study involves three major steps (\fig\ref{fig:MethodologyOverall}):
\begin{enumerate}
  \item \bf{Data Collection}: We collect posts where reputation fraud scenarios are discussed.
  \item \bf{Data Analysis}: We manually label reputation fraud scenarios discussed in the posts.
  \item \bf{Fraud Scenario Report}: We report the fraud scenarios by connecting those with specific examples from the posts.
\end{enumerate} We discuss the steps below.

\nd\bf{$\bullet$ Data Collection.} We are aware of no previous research that specifically looked into the fraudlent behaviors of Stack Overflow uers 
to exploit the reputation mechanisms. Stack Overflow also does not share information about the reputation fraud scenarios. 
Therefore, in the absence of any specific guidelines or a particular dataset, we attempt to learn about the reputation fraud scenarios 
from the discussions of developers in two Stack Overflow meta sites: meta.stackoverflow.com and meta.stackexchange.com. 
StackExchange is the parent site for the online developer forum Stack Overflow. Stack Exchange consists of a network 
of online Q\&A sites, including Stack Overflow. StackOverflow is the most actively-viewed site
in the network. Each StackExchange site contains a \it{meta} sub-site where
users consult rules/issues. We picked the two meta-sites because they
feature programming discussions and the two meta sites are the most popular sites among all meta sites in Stack Exchange network.


On 9 March 2018, we searched the sites using the query
`voting+ring'. We picked this search query, because in our informal analysis of Stack Overflow posts, we found that 
this pharse is commonly used to denote different
reputation frauds. The query returned 8,553 posts (4,265 from meta.stackexchange.com, 4,286
from meta.stackoverflow.com).
The posts contained discussions from 1,728
distinct users, 25 of them participated in both sites.
%The average score\Foutse{explain what this score is! and what it means...} of
% the posts was 6.2 (maximum 1224).
From the 8,553 posts, we randomly picked 1,697 posts. This
subset is a statistically significant representation of the 8553 posts with a 99\% confidence interval.


\nd\bf{$\bullet$ Data Analysis.} We manually analyzed each post to determine whether the post contains discussion about a reputation 
fraud scenarios and if so (i.e., it contains), we give the type of fraud scenario a name by reading the contents of the post. 
To do the analysis, we use open card sorting. Specifically, our card sorting approach attempted to categorize each of the 1697 posts as follows:
\begin{enumerate}%[style=nextline]
\item\bf{Scenario.}{The post discusses a reputation fraud scenario. If so, we give the scenario a name by analyzing the scenario type as discussed in the post contents.}
%\item[Solution.]{Discusses a solution to a reputation fraud scenario}
\item\bf{Concerns}{The post discusses relevant information but not a reputation fraud scenario, e.g., developers' concerns.}
\item\bf{Irrelevant.}{The post contents are not related to any reputation fraud scenaio.}
\end{enumerate}

%
% We load and preprocess our dataset from Stack Overflow to analyze the
% fraud scenarios in two steps: \begin{inparaenum}[(1)]
% \item We find a total of 8553 posts from Stack Overflow that discuss
% reputation fraud scenarios involving different types of voting rings.
% \item In the absence of any previous studies conducted to understand reputation fraud
% scenarios in developer forums, it was necessary for us to manually verify the
% type of contents discussed in the forum posts where reputation frauds are
% discussed. From the 8553 posts, we randomly picked a statistically significant
% subset of 1697 posts. We manually annotated each post
% by the type of content (e.g., type of scenario mentioned, the solutions
% discussed).
% \end{inparaenum}
%
% \subsection*{Step 1. Data Loading}

% We searched these two sites for threads related to
% reputation fraud on March 9, 2018. We leveraged the search engine of the sites
% and used the query `voting ring'. We picked this query because any reputation
% fraud in the network involves a \it{ring} of developers/users who commit the
% fraud by placing their vote in different ways. The query returned a
% total of 8553 posts from 203 threads (4265 posts from meta.stackexchange.com and 4286
% from meta.stackoverflow.com). The posts contained discussions from a total of
% 1728 distinct users. The average score\Foutse{explain what this score is! and what it means...} of the posts was 6.2 (maximum 1224).
%
The categorization involved five
steps:
\begin{enumerate}
  \item \bf{Coding Consultation.} The two authors consulted 97 posts together to
  prepare coding guide.
  \item \bf{Reliability Analysis.} The authors then separately coded 58 additional posts.
  The percent agreement between them was 83.3\%, which was substantial (Cohen $\kappa=.632$).
  \item \bf{Coding Completion.} With substantial agreement level, we
  assumed that either of the authors can label other
  posts. The first author labeled other posts.
  \item \bf{Clustering.} The labels are revisited multiple times to finalize their coding and to group the scenarios into higher categories.
  \item \bf{Finalize Coding.} The two authors discuss together the overall coding and the list of final reputation fraud scenarios.
\end{enumerate} 



\nd\bf{$\bullet$ Fraud Scenario Report.} We report the reputation fraud scenarios by triangulating, i.e., by connecting each fraud scenario to the list of posts where the fraud scenario 
was discussed. We report the distribution of each scenario in the posts. In addition, we draw flowchart of each scenario to explain the roles of each participating user in the scenario (e.g., 
fraud user vs a victim of fraud scenario).

\subsection{Study 2. Detection of Suspicious Reputation Frauds}
In our second study, we attempted to automatically detect suspicious reputation in Stack Overflow. 
Stack Overflow does not share information about reputation frauds. Stack Overflow also removes 
several fields in its data dumps that are needed to detect reputation frauds, the tracking of upvotes and downvotes to a post (e.g., who downvoted to post and when the downvoted happened). 
Stack Overflow also removes suspicious posts in Stack Overflow using its internally developed scripts. However, we observed that while Stack Overflow removes 
posts that are suspicious and removes the corresponding scores from a suspicious user, the user record is not deleted. Therefore, we cannot detect algorithms to find such reputation frauds explicitly in Stack Overflow. To detect the suspicious reputation frauds, we proceeded with the follow three major steps.
\begin{enumerate}
  \item \bf{Identify Algorithm Design Requirements.} We identify the algorithm design requirements by focusing on two things: the key characteristics of the reputation frauds, and the availability of public data in Stack Overflow 
  as required for us to detect the reputation frauds.
  \item \bf{Develop Algorithm.} We develop two algorithms to detect the reputation frauds who attempt to exploit the reputation mechanisms to gain their reputation scores.
  \item \bf{Evaluate Algorithm.} We evaluate the two algorithms by taking a sample of Stack Overflow users that are labeled as suspicious by our algorithms.
\end{enumerate} We discuss the steps below.

\nd\bf{$\bullet$ Identify Algorithm Design Requirements.} Given that the primary motivation for reputation frauds is to increase their reputation scores, we focused on developing algorithms to identify users whose reputation scores have 
shown significant increase over time. To understand the specific characteristics of such users, we analyzed 50 randomly selected 
questions in Stack Overflow where 
the identification behavior of such users are discussed by other Stack Overflow users. The first and second authors 
discussed in multiple collaborative sessions about the indicators discussed in the posts. 
The final list of indicators are then used to develop heuristics for the algorithms to detect suspicious reputation frauds.
  
\nd\bf{$\bullet$ Develop Algorithms.} By repeated analyses of the 
indicators, we identified two major traits of the reputation frauds: they often work in small community and they show 
abnomral jump in their reputation scores over time. We thus developed two algorithms based on the two traits. 
Both of our proposed algorithms use the publicly available data in Stack Overflow dumps. Therefore, our algorithms 
do not require the information of how each post is upvoted or downvoted and by whom. As we noted above, such sensitive information are not shared by Stack Overflow. 
Our first algorithm detects suspicious community of users who show high degree (i.e., frequency) and intensity (i.e., in very short time) of interactions among 
the users in the community. Our second algorithm simply finds users whose reputation scores showed unusual jump in a short time. 

\nd\bf{$\bullet$ Evaluate Algorithms.} We evaluated the two algorithms by downloading the entire history of reputation logs of each user that is 
considered as suspicious by our two algorithms. Stack Overflow online site provides a dashboard for each user to show how each activity of a user resulted in 
the increase or decrease of reputation score of a user. Once a user gains a reputation score, Stack Overflow can remove the score, if the process to gain the reputation 
was not recommended (i.e., due to a suspicious activity). In a total of 10 different configurations of our two algorithms (e.g., varying the threshold of jump in reputation score for algorithm 2), 
we find that our algorithms can find such suspicious reputation frauds with 60-90\% accuracy. The two algorithms offer largely superior performance than 
a `Random Walk' algorithm that randomly labels a Stack Overflow user as suspicious.  
